Population-Dependent r-process Scatter in the Globular Cluster M15

Multiple populations, defined by correlations between light element abundances, are an almost ubiquitous property of globular clusters. On the other hand, dispersions among the heavy elements are limited to a few rare clusters. In this letter, we present Mg, Y, Ba, La, and Eu measurements for 89 stars in M15 with errors < 0.4 dex from Keck/DEIMOS medium-resolution spectra. We find higher Ba, La, and Eu dispersions in the first generation of stars than in the second generation at a significance of $\ge$2 $\sigma$. This is evidence for inhomogeneous mixing of gas during the formation of the first generation of stars, which subsequently became well-mixed prior to the formation of the second generation of stars. If the r-process event that caused the abundance dispersions was born with the first population of stars, it must be an r-process site with a short delay time.

==> tab1example.tex <==
% \movetabledown=3.8in
\begin{deluxetable}{cccccccccc}
\tablecaption{Multi-Element Abundance Catalog of M15 Stars \label{tab:abundances}}
\tablehead{\colhead{Name} & \colhead{S/N blue} & \colhead{Temp (K)} & \colhead{$\log g$} & \colhead{[Fe/H]} & \colhead{[Mg/Fe]} & \colhead{[Y/Fe]} & \colhead{[Ba/Fe]} & \colhead{[La/Fe]} & \colhead{[Eu/Fe]}}
\startdata
51057 & 50.49 & 4707 & 1.47 & -2.65$\pm$0.02 & $+0.58^{+0.01}_{-0.01}$ & $-0.20^{+0.03}_{-0.04}$ & $+0.16^{+0.02}_{-0.02}$ & $+0.01^{+0.04}_{-0.07}$ & $+0.40^{+0.03}_{-0.22}$ \\[2mm]
50051 & 50.33 & 4996 & 1.65 & -2.68$\pm$0.04 & $+0.71^{+0.03}_{-0.03}$ & $-0.09^{+0.09}_{-0.14}$ & $+0.32^{+0.08}_{-0.06}$ & \nodata & $+0.52^{+0.15}_{-0.50}$ \\[2mm]
38026 & 60.85 & 4436 & 0.63 & -2.44$\pm$0.02 & $+0.65^{+0.01}_{-0.01}$ & $-0.18^{+0.03}_{-0.05}$ & $+0.25^{+0.02}_{-0.04}$ & $+0.30^{+0.03}_{-0.03}$ & $+0.58^{+0.03}_{-0.09}$ \\[2mm]
49658 & 74.51 & 4611 & 1.26 & -2.56$\pm$0.02 & $+0.58^{+0.01}_{-0.01}$ & $-0.10^{+0.03}_{-0.10}$ & $+0.30^{+0.03}_{-0.04}$ & $+0.53^{+0.05}_{-0.05}$ & $+0.78^{+0.09}_{-0.25}$ \\[2mm]
60808 & 20.27 & 4546 & 1.20 & -2.54$\pm$0.01 & $+0.51^{+0.01}_{-0.02}$ & $-0.32^{+0.08}_{-0.02}$ & $+0.31^{+0.01}_{-0.18}$ & $+0.34^{+0.02}_{-0.04}$ & $+0.87^{+0.05}_{-0.05}$ \\[2mm]
66116 & 43.55 & 6106 & 2.83 & -2.45$\pm$0.08 & $+0.80^{+0.04}_{-0.06}$ & $<+0.34$ & $+0.34^{+0.09}_{-0.15}$ & $+1.55^{+0.11}_{-0.22}$ & $<+1.76$ \\[2mm]
61191 & 36.46 & 5359 & 2.87 & -2.40$\pm$0.05 & $+0.42^{+0.02}_{-0.04}$ & $+0.22^{+0.09}_{-0.18}$ & $+0.54^{+0.09}_{-0.08}$ & $+1.17^{+0.09}_{-0.08}$ & $+1.16^{+0.13}_{-0.48}$ \\[2mm]
16135 & 78.27 & 4695 & 0.47 & -2.68$\pm$0.01 & $-0.12^{+0.08}_{-0.01}$ & $-0.14^{+0.14}_{-0.01}$ & $+0.34^{+0.01}_{-0.03}$ & $+0.18^{+0.09}_{-0.02}$ & $+0.69^{+0.04}_{-0.05}$ \\[2mm]
7815 & 59.94 & 6217 & 3.15 & -2.81$\pm$0.21 & $+0.68^{+0.07}_{-0.18}$ & $<+0.96$ & $+0.02^{+0.28}_{-0.44}$ & \nodata & \nodata \\[2mm]
49428 & 110.85 & 4828 & 1.60 & -2.63$\pm$0.02 & $+0.20^{+0.02}_{-0.02}$ & $-0.06^{+0.05}_{-0.03}$ & $+0.37^{+0.02}_{-0.04}$ & $+0.36^{+0.05}_{-0.04}$ & $+0.66^{+0.05}_{-0.10}$ \\[2mm]
11998 & 88.34 & 5486 & 3.39 & -2.51$\pm$0.06 & $+0.47^{+0.02}_{-0.04}$ & $<+0.15$ & $+0.01^{+0.06}_{-0.16}$ & \nodata & \nodata \\[2mm]
49479 & 52.15 & 4697 & 1.37 & -2.57$\pm$0.02 & $+0.61^{+0.02}_{-0.01}$ & $-0.37^{+0.08}_{-0.12}$ & $-0.02^{+0.06}_{-0.05}$ & $<-0.14$ & $+0.38^{+0.11}_{-0.21}$ \\[2mm]
57577 & 50.29 & 4797 & 1.63 & -2.52$\pm$0.03 & $+0.63^{+0.02}_{-0.02}$ & $+0.12^{+0.05}_{-0.11}$ & $+0.42^{+0.04}_{-0.08}$ & $+0.60^{+0.04}_{-0.09}$ & $+1.08^{+0.10}_{-0.09}$ \\[2mm]
30961 & 79.20 & 4339 & 0.56 & -2.49$\pm$0.03 & $+0.51^{+0.02}_{-0.01}$ & $-0.39^{+0.10}_{-0.02}$ & $-0.21^{+0.04}_{-0.02}$ & $+0.12^{+0.04}_{-0.04}$ & $+0.58^{+0.03}_{-0.06}$ \\[2mm]
56734 & 66.14 & 4639 & 1.28 & -2.52$\pm$0.02 & $+0.58^{+0.02}_{-0.01}$ & $-0.19^{+0.06}_{-0.06}$ & $+0.31^{+0.03}_{-0.05}$ & $+0.40^{+0.03}_{-0.07}$ & $+0.69^{+0.09}_{-0.17}$ \\[2mm]
55914 & 87.29 & 4664 & 1.32 & -2.60$\pm$0.01 & $+0.53^{+0.01}_{-0.01}$ & $-0.13^{+0.07}_{-0.04}$ & $+0.41^{+0.01}_{-0.03}$ & $+0.53^{+0.01}_{-0.12}$ & $+0.91^{+0.01}_{-0.36}$ 
\enddata
\tablecomments{Stellar parameters and abundances for a subset of M15 stars in this study. A full version of this table, including coordinates and upper limits, is available in a machine-readbale format. S/N blue is the signal-to-noise of the blue spectrum (900ZD or 1200B), where most of the neutron-capture absorption lines are located.}
\end{deluxetable}

